Improving Generalization Ability of Robotic Imitation Learning by Resolving Causal Confusion in Observations

Recent developments in imitation learning have considerably advanced robotic manipulation. However, current techniques in imitation learning can suffer from poor generalization, limiting performance even under relatively minor domain shifts. In this work, we aim to enhance the generalization capabilities of complex imitation learning algorithms to handle unpredictable changes from the training environments to deployment environments. To avoid confusion caused by observations that are not relevant to the target task, we propose to explicitly learn the causal relationship between observation components and expert actions, employing a framework similar to [6], where a causal structural function is learned by intervention on the imitation learning policy. Disentangling the feature representation from image input as in [6] is hard to satisfy in complex imitation learning process in robotic manipulation, we theoretically clarify that this requirement is not necessary in causal relationship learning. Therefore, we propose a simple causal structure learning framework that can be easily embedded in recent imitation learning architectures, such as the Action Chunking Transformer [31]. We demonstrate our approach using a simulation of the ALOHA [31] bimanual robot arms in Mujoco, and show that the method can considerably mitigate the generalization problem of existing complex imitation learning algorithms.

==> scratch.tex <==
% \red{THE SUBMISSION IS LIMITED TO 9 CONTENT PAGES}
% \paragraph{Points to be addressed}
% \begin{itemize}
% \item Generalization/distribution shift problem is severe in robotic imitation learning algorithms, e.g., ACT and HIT.
% \item Representation requirement in \cite{de2019causal} does not applicable in robotic imitation learning.
% \item CNN output is ubiquitously accessible in robotic imitation learning pipelines, and is an easily obtainable feature representation.
% \item Correlation between (Resenet-18) features is not an issue for constructing the underlying causal model, but the main challenge is the large graph sampling space.
% \end{itemize}
% The contributions of this work are: ...
%% (hot) lead in what is IL and why it matters
% Imitation learning allows learning from expert demos

% In this section we present relevant works that explain the context of our work and the existing limitations of existing approaches.
% \paragraph{Machine Learning in Robotic Manipulation.}
% % What is ML and how it is used for manipulation
% A core objective of robotic manipulation is to enable systems to perform complex tasks, requiring policies that select appropriate actions based on the current observation. 
% % Different types of ML we care about
% Machine learning has been a crucial development in this field and has a diverse array of approaches, including reinforcement learning~\cite{haarnojaSoftActorCritic2018, kalashnikovScalableDeep2018,levineEndtoEndTraining2016}, supervised methods~\cite{pintoSupersizingSelfsupervision2016, lynchLearningLatent2019}, and hybrid approaches~\cite{zhaoHybridLearning2022, shridharCLIPortWhat2022}. 
% % what have they been used for
% These approaches have been successfully used to complete a range of tasks(\red{citations needed, left open for papers people want to put here}). 
% % what are their limitations (setup for where our work fits in)
% However, they often suffer from limited generalization, require large amounts of training data, require explicitly defined reward functions, and are sensitive to distribution shifts between their training and deployment environment~\cite{dulacarnoldChallengesRealworld2021, levineOfflineReinforcement2020}.

%
% % Large scale data gathering improves generalization
% Several strategies have been explored to address the generalization of machine learning models. One dominant approach is large-scale data collection from a diverse set of real-world environments that the system may encounter, such as in: \cite{zhao2024aloha, o2024open}
% % but its expensive
% Although these techniques can be effective, these methods are highly resource-intensive, they can require substantial time, money, computational power and human labor which makes them impractical or impossible for many applications.
% % people try similar things in simulation
% An alternative approach to large-scale real-world data collection is the use of simulated environments to augment or replace real-world data. Common strategies are domain randomization (DR)~\cite{tobinDomainRandomization2017, makoviychukIsaacGym2021, anderson2021sim} and generative simulation methods~\cite{jamesSimToRealSimToSim2019}.
% % what is DR
% DR randomizes parameters of the simulation with the aim of encouraging models to learn more robust features or features that are invariant between the varying conditions -- suggesting that they are task-relevant. In particular, DR varies parameters such as lightning, object positions, textures, and friction. 
% % DR limitations (set up for the comparisons we make in the results (needs many sample, still weak to domain shift if you dont model it)
% However, the quality of the learned models strongly depends on the chosen tuning parameters, quality and quantity of the simulated data~\cite{prakashStructuredDomain2019}, costs additional computational resources~\cite{openaiSolvingRubiks2019}, and can result in overly conservative behaviors due to the broad task and environment distributions~\cite{zhao2020sim}.
% This results in methods that are fragile in different ways and are computationally expensive to train due to their sample inefficiency.


% Causal methods have been proposed as a technique to improve the robustness and generalization ability of learning-based methods by modeling the causal relationships between observations and actions~\cite{Pearl2000causal, peters2017elements}. 
% Doing this allows these methods to distinguish which features are actually relevant and predictive rather than spurious correlations.
% This allows the learners to avoid incorrectly overfitting to patterns observed in the training data, that are irrelevant to the actual task and deployment.
% By utilizing these causally-relevant features sample efficiency is increased and the models become more robust to domain shifts~\cite{yaoSurveyCausal2021}. This technique has seen recent success in machine learning tasks such as visual prediction~\cite{zengTransporterNetworks2021}, reinforcement learning~\cite{zhang2020invariant} and imitation learning~\cite{de2019causal}.
% These causal approaches are promising because they are structured and they can help alleviate some of the high cost of gathering diverse real-world data.

% which have been shown to perform well due to the attention mechanisms enabling modeling of temporal components.
% Furthermore, methods that utilize `action chunking' have been shown to further improve performance in manipulation tasks~\cite{zhao2023learningACT, black2410pi0}.
% Although they can deal with variance in the training data and some perturbations in the environment during deployment they still are vulnerable to large enough domain discrepancies~\cite{zareSurveyImitation2024}.

% While effective in simple scenarios it introduces inductive biases~\cite{locatello2019challenging} and is non-trivial to learn for complex robotic manipulation settings with high-dimensional observations and large coupled action spaces. and integrates causal structure learning to a transformer-based imitation learning architecture like ACT~\cite{zhao2023learningACT}. We demonstrate improved generalization to out-of-distribution scenarios without relying on extensive data collection (simulated or real) through improved sample efficiency. Our work bridges a crucial gap between causal inference methods and practical robotic applications.   

% In this work, we identify and address the problem of causal confusion in imitation learning (IL), where models learn spurious correlations in observations that do not effect the actual causal structure of the expert demonstrations. This issue is particularly an issue when the IL model experiences an environment dissimilar from its trained conditions, where these irrelevant features no longer exist and performance is degraded.

% We show in contrast to previous work that learning causal structures in IL does not need disentangled representations. Using this insight we propose Causal-ACT, an effective extension to a transformer-based IL model that includes causal structure learning in the training process. By optimizing the causal graph our method focuses on the components that are important to task success and demonstrates improved generalization to new environments. We justify these results theoretically and empirically through simulation showing a substantial improvement over the ACT baseline and improved sampled efficiency compared to domain randomization.

% In future work, we plan to extend this framework to other imitation learning architectures besides ACT and evaluate its effectiveness against a broader set of manipulation tasks in real-world environments. Additionally we want to explore other classes of causal structure learning and see if they yield further improvements to generalization of IL techniques. 

